Fixed Confidence Best Arm Identification in the Bayesian Setting

We consider the fixed-confidence best arm identification (FC-BAI) problem in the Bayesian setting. This problem aims to find the arm of the largest mean with a fixed confidence level when the bandit model has been sampled from the known prior. Most studies on the FC-BAI problem have been conducted in the frequentist setting, where the bandit model is predetermined before the game starts. We show that the traditional FC-BAI algorithms studied in the frequentist setting, such as track-and-stop and top-two algorithms, result in arbitrarily suboptimal performances in the Bayesian setting. We also obtain a lower bound of the expected number of samples in the Bayesian setting and introduce a variant of successive elimination that has a matching performance with the lower bound up to a logarithmic factor. Simulations verify the theoretical results.

==> sections/lower_bound.tex <==
\section{Lower bound}\label{sec:lower bound}

%\junpei{modified: First contribution is preliminary section (Freq $\delta$-correct algorithm has indefinite Bayesian stopping time)}
This section will elaborate on
%on our first main contribution, which is
the lower bound of the stopping time in the Bayesian setting. 
Theorem \ref{thm: main lower bound} {below} states that any Bayesian $(\bH, \delta)$-correct algorithm requires the expected stopping time of at least $\Omega(\frac{L(\bH)^2}{\delta})$. 
%\kazu{We may want to avoid calling it ``stopping time" as ``stopping time" has its own meaning in probability theory. ``sample size" instead?}
%Formally, it can be expressed as follows.
\begin{thm}\label{thm: main lower bound}
    {Define $\sigma_{\min} = \min_{i \in [k]} \sigma_i^2$ and $N_V = \frac{ L(\bH)^2 \sigma_{\min}^2 \ln 2}{8e^4 \delta}$.} For any BAI algorithms $\pi=((A_t), \tau, J)$ and sufficiently small\footnote{$\delta<\delta_0 (\bH):= $} $\delta$, {if} $ \Ex_{\bmu \sim \bH} [\tau] \leq N_V$, then $\mathrm{PoE}(\pi;\bH) \geq \delta$. 
\end{thm}
In this main body, we will use the two-armed Gaussian bandit model with homogeneous variance condition (i.e. $\sigma_1 = \sigma_2 = \sigma$) for easier demonstration of the proof sketch.
{Theorem \ref{thm: main lower bound}, which is more general in the sense that it can deal with $k>2$  arms with heterogeneous variances, is proven in Appendix \ref{appsec: lower bound}.} 

% \junpei{We obtain an optimization that lower-bounds the probability of error with constraints on the expected stopping time $N_V$ (Opt 2), which gives a minimum value of $N_V$ such that we can have the PoE smaller than $\delta$.}
%\junpei{I guess informal discussion suffices for $k=2$, or we should say that the following line is essentially the same as the formal proof for general $k$.}
%\junpei{Can we shorten the lower bound proof? It is currently 1+1/4 pages, which is a bit long.}
\paragraph{Sketch of the proof, {for $k=2$:}} It suffices to show that the following is an empty set:
\[
\mathcal{A}^b (\delta, \bH, N_V) := \{ \pi \in \mathcal{A}^b (\delta, \bH): \Ex_{\bmu \sim \bH} [\tau] \leq N_V\}.
\]

Assume that $\mathcal{A}^b (\delta, \bH, N_V) \neq \emptyset$ and choose an arbitrary $\pi \in \EA^b (\delta, \bH, N_V)$. We start from the following transportation lemma:

\begin{lem}[\citealt{kaufman16a}, Lemma 1]\label{lem_transportation_lemma} Let $\delta \in (0, 1)$. For any algorithm $((A_t), \tau, J)$, any $\EF_\tau$-measurable event $\EE$, any bandit models $\bmu, \blambda \in \{(x,y)\in \mathbb{R}^2: x\neq y\}$ such that $i^*(\bmu) \neq i^*(\blambda)$, 
\begin{equation*}
    \Ex_{\bmu} \bracket{\sum_{i=1}^2 \mathrm{KL}_i(\mu_i, \lambda_i) N_i (\tau)} \geq d(\Prob_{\bmu} ({\EE}), \Prob_{\blambda} ({\EE})).
\end{equation*}
\end{lem}
Note that the above Lemma holds for any algorithm, so the above theorem works for any stopping time $\tau$. Now define $\bnu (\bmu)$ as a swapped version of $\bmu \in \mathbb{R}^2$, which means $(\bnu(\bmu))_1 =\mu_2, \bnu(\bmu)_2 = \mu_1$, and let $\EE = \{J \neq i^* (\bmu)\}$, the event that the recommendation of the algorithm is wrong. Substituting $\blambda$ with $\bnu(\bmu)$ from the above equation of Lemma \ref{lem_transportation_lemma} leads 
\begin{align*}
    \Ex_{\bmu} \bracket{\frac{(\mu_1-\mu_2)^2}{2\sigma^2} \tau} &\geq d(\PoEPair (\pi;\bmu),1-\PoEPair (\pi;\bnu)) \geq \log \frac{2}{2.4 (\PoEPair (\pi;\bmu)+\PoEPair(\pi;\bnu))}. 
\end{align*}
Note that the first inequality comes from the fact that $\EE$, the failure event of the bandit model $\bmu$, is exactly a success event of the bandit model $\bnu(\bmu)$ in this two-armed case, and the last inequality is from Eq. (3) of \cite{kaufman16a}. One can rewrite the above inequality as
\begin{equation}\label{eqn:modified_transportation_lemma}
    \frac{\PoEPair (\pi;\bmu)+\PoEPair(\pi;\bnu)}{2} \geq \frac{1}{2.4}\exp\paren{\Ex_{\bmu} \bracket{- \frac{(\mu_1 - \mu_2)^2}{2\sigma^2} \tau}}.
\end{equation}
% Now, the objective of this proof is to check how small $\mathrm{PoE} (\pi;\bH)$ could be with an optimal algorithm when the expected number of samples is bounded by $N_V$. Suppose that an algorithm $\tilde{\pi}=((A_t), \tau, J)$ has $\PoEPair (\bH)\leq \delta$ and satisfies $\Ex [\tau] \brown{\Ex_{\bmu \sim \bH} [\tau] ?} \leq N_V$. 

% \kazu{How about defining this set of strategies 
% \[
% \mathcal{A}^b (\delta, \bH, N_V) = \{ \pi \in \mathcal{A}^b (\delta, \bH): \Ex_{\bmu \sim \bH} [\tau] \leq N_V\}
% \]
% Then, we argue for all $\pi \in \mathcal{A}^b (\delta, \bH, N_V) $
% \[
% \textrm{PoE}(\pi, \bH) \geq V_0(\pi, \bH) \geq V_0 \geq V' \geq \delta
% \]
% leading a condtradiction. Thus, $\mathcal{A}^b (\delta, \bH, N_V) = \emptyset$, which is what we want?
% }
We can rewrite the conditions of $\mathcal{A}^b (\delta, \bH, N_V)$ as
\begin{align*}
    \PoEPair (\pi;\bH)&=\int_{\bmu \in \mathbb{R}^2} \PoEPair (\pi;\bmu) \diff \bH (\bmu) \leq \delta \qquad
    \text{and } & \int_{\bmu \in \mathbb{R}^2} \Ex_{\bmu} \bracket{\tau} \diff \bH (\bmu) \leq N_V. \tag{Opt0}
\end{align*}
Using Eq. \eqref{eqn:modified_transportation_lemma} {and with some symmetry tricks}, we get $V_0 \leq \PoEPair (\pi;\bH)$ where
\begin{align}\label{eqn:strategy condition}
    V_0 := \int_{\bmu \in \mathbb{R}^2} \frac{1}{2.4} \exp {\paren{-\frac{(\mu_1 -\mu_2)^2}{2\sigma^2}\Ex_{\bmu} \bracket{\tau}}} \diff \bH (\bmu) \leq \delta 
    \ \text{ and } \int_{\bmu \in \mathbb{R}^2} \Ex_{\bmu} \bracket{\tau} \diff \bH (\bmu) \leq N_V. \tag{Opt1}
\end{align}
Note that on the above two inequalities, only $\Ex_{\bmu}[\tau]$ is the value that depends on the algorithm $\pi$. Now our main idea is that we can relax these two inequalities to the following optimization problem by substituting $\Ex_{\bmu}[\tau]$ to an arbitrary $\tilde{n}: \mathbb{R}^2 \to [0,\infty)$ as follows:
\begin{align}\label{eqn:opt1}
    V := \inf_{\tilde{n}:\mathbb{R}^2\to [0,\infty)} \int_{\bmu \in \mathbb{R}^2} \exp {\paren{-\frac{(\mu_1 -\mu_2)^2}{2\sigma^2}\tilde{n}(\bmu)}} \diff \bH (\bmu)\ 
    \text{ s.t. } \int_{\bmu \in \mathbb{R}^2} \tilde{n}(\bmu) \diff \bH (\bmu) \leq N_V \tag{Opt2}
\end{align}
and $V\leq 2.4 V_0 \leq 2.4\delta$. {Let $\EN:= \{ \bmu \in \mathbb{R}^2: |\mu_1 - \mu_2|<\Delta:=\frac{8\delta}{L(\bH)}\}$. From the discussions in Section \ref{subsec: two armed gaussian}, one might notice that $\EN$ is an important region for bounding $\Ex_{\bmu \sim \bH}[\tau]$.} We can relax the above \eqref{eqn:opt1} to the following version, which focuses more on $\EN$:
\begin{align}\label{eqn:opt2}
    V' := \inf_{\tilde{n}:\mathbb{R}^2\to [0,\infty)} \int_{\bmu \in \EN} \exp {\paren{-\frac{(\mu_1 -\mu_2)^2}{2\sigma^2}\tilde{n}(\bmu)}} \diff \bH (\bmu) 
    \text{ s.t. } \int_{\bmu \in \EN} \tilde{n}(\bmu) \diff \bH (\bmu) \leq N_V. \tag{Opt3}
\end{align}
One can prove $V'\leq V \leq 2.4 \delta$. Now, if we notice that function $x \mapsto \exp {\paren{-\frac{(\mu_1 -\mu_2)^2}{2\sigma^2}x}}$ is a convex function, we can use Jensen's inequality to verify that the optimal solution for \eqref{eqn:opt2} is when $\tilde{n} = \frac{N_V}{\Ex_{\bmu \sim \bH} \bracket{\Ind_\EN}} \Ind_{\EN}$, and when we use $N_V$ in Theorem \ref{thm: main lower bound}, one can get: 
\begin{align}
{V'}&\ge \int_{\bmu \in \EN}
\exp\left(-\frac{\Delta^2}{2\sigma^2}\cdot \paren{\frac{N_V}{\EE_{\bmu \sim \bH}[\Ind_{\EN}]}} \right) 
d\bH(\bmu) \tag{by optimality of $\tilde{n} = \frac{N_V}{\Ex_{\bmu \sim \bH} \bracket{\Ind_\mathcal{N}}}$} \\
&\geq \int_{\bmu \in \EN}
\exp\left(-\frac{\Delta^2 \cdot N_V }{\sigma^2 \Delta L(\bH)}\right) 
d\bH(\bmu) \geq \exp\left(-\frac{\Delta \cdot N_V }{\sigma^2 L(\bH)}\right) \cdot \Delta L(\bH) \tag{both by Lemma \ref{lem:volume_lem}}\\
&> 2.4\delta \tag{by definition of $N_V$ and $\Delta$}, 
\label{ineq:poe_as_draw}
\end{align}
which is a contradiction. 
This means no algorithm satisfies \eqref{eqn:strategy condition}, and the proof is complete. 

==> sections/related_works.tex <==
\section{Related Work}

\junpei{I moved related work before the problem setup. It may be at the end of the paper. Also, it is not necessary in my view but for some reason CS people like is in favor of related work section...}

\junpei{We want to mention $\epsilon$-best answer identification papers because it is the most close to our algorithms.}


\begin{table}[h]
\caption{Position of our algorithm in BAI}
\label{table:position of our algorithm}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|cc}
\toprule
& \multicolumn{2}{c}{Approach}\\ %maybe better word than approach?
Objective & Freq. & Bayes \\
\midrule
Fixed Confidence    &  \cite{garivier16,kaufmann2016complexity, qin2017improving,Russo2016, jourdan2022top}& Ours\\
Fixed Budget & \cite{komiyama2022minimax, komiyamakkc_bayesian}& \cite{atsidakou2023bayesian}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\paragraph{Best-Arm Identification (BAI)} As mentioned in the introduction, extensive research has been conducted on BAI in the Frequentist setting where the learner assumes a fixed $\bmu$ before the start of the game. For instance, in the fixed confidence setting, \cite{garivier16,kaufmann2016complexity, qin2017improving} provided lower bounds on stopping time and presented asymptotically optimal algorithms for best-arm identification. \cite{Russo2016, jourdan2022top} conducted in-depth analyses in Bayesian algorithms, but the performance of their algorithm is based on the frequentist setting. \cite{DBLP:conf/ciss/JamiesonN14} thoroughly summarizes this fixed-confidence BAI in the Frequentist setting. 
\junpei{The distinction between FC and FB is made by \cite{Carpentier2016}. \cite{komiyama2022minimax} describe minimax-optimal performance for FB-BAI.}
\junpei{\cite{atsidakou2023bayesian} is a subsequent research of mine \cite{komiyamakkc_bayesian} (appeared earlier).}
In the fixed budget setting, \cite{komiyama2022minimax} demonstrated meaningful distinctions from the fixed confidence setting and proposed novel algorithms. However, many of the aforementioned studies focused on the Frequentist setting, and research on the Bayesian setting, where instances are sampled from priors, was limited to \cite{atsidakou2023bayesian} in the fixed budget setting. 
To the best of our knowledge, we are the first to investigate the Bayesian setting and fixed confidence setting concurrently.

\paragraph{Ranking and Selection (R\&S)} Ranking and selection is another topic that is deeply related to BAI since they both rank the possible options and select the best option eventually \cite{mcdonald1998conversation,bechhofer1954single}. R\&S also have a fixed-budget setting and fixed-confidence setting in their problem setting. We recommend \cite{hong2021review} for an overall review of this field. As researchers of \cite{hong2021review} have mentioned, the main difference between the two is that BAI assumes sub-gaussian distributions with known sub-gaussian proxy upper bound of arms while R\&S assumes reward distributions of arms as Gaussian with unknown variance. 
\junpei{These arguments are 80\% correct, but too strong to state without reservation. Let me see...}
Plus, in the fixed-confidence setting, many papers focus more on probability guarantee when the algorithm terminates, rather than the expected stopping time itself. Because of these technical differences, many R\&S studies omitted the expected stopping time argument, or proved their performance by simulations rather than theoretical proof of expected stopping time \cite{kim2006asymptotic, kim2006selecting, qu2012ranking,bowen2022bayesian, gorder2019ranking}. In our paper, our main objective is to minimize the expected stopping time. 

We also want to point out that we are also using a similar trick of the R\&S called the 'indifference zone' strategy for our algorithm. This strategy is basically when the difference of the mean between the best arm and a sub-optimal arm is too small, then we will regard them as indifferent. This trick is not new in FC-BAI - \cite{jourdan2023varepsilon} used this $\epsilon$-indifferent criterion for the FC-BAI problem in the Frequentist setting. 

\paragraph{Bayesian Design} In multi-armed bandit (MAB), which can be considered a close relative to Best Arm Identification (BAI), extensive research has been conducted on Bayesian design, with the introduction of the term Bayesian regret for analyzing algorithm performance \cite{lattimore2016regret, russo2014learning, lattimore2020bandit}. However, while the goal of BAI is the accuracy of the final recommendation after all sampling, MAB aims to minimize cumulative regret, which is the difference from the optimal at each sample. As their objectives differ, the forms of algorithms in these two fields are somewhat distinct.


\begin{comment}
\begin{easylist}
@ Gabilon's unified algorithm \ref{GabillonGL12}.
@ Jamieson's survey \cite{DBLP:conf/ciss/JamiesonN14}.
@ May describe related work in R\&S if there are Bayesian stopping. 
@@ cite Kazutoshi's work. 
@@ In my view, OR lit put less emphasis on the sampling rule and less emphasis on the uncertainty of the model parameters.
@ Did recent results (such as Assaf Zeevi's ICML paper) describe Bayesian performance?
\end{easylist}

% What KG / Information-directed sampling guarantee?
% IDS https://arxiv.org/pdf/1403.5556.pdf

Discusses the Bayesian FB-BAI results \cite{komiyamabsr,atsidakou2023bayesian}. We consider FC-BAI to be more interesting mainly because the difference between frequentist best and Bayesian best algorithms is more pronounced in our fixed-confidence case.

Recent work of Marc Jourdan on $\eps$-insensitive BAI? \cite{jourdan2023varepsilon}. They proposed an anytime algorithm $\text{EB-TC}_\epsilon$, which is leader-challenger type algorithm. 
%Junpei: read very quickly. 
% recommendation rule: empirical best arm
% selection rule: I have not fully checked yet, but it seems that this is not early stopping type alg.
\end{comment}
